A Comparison of Bayesian Prediction Techniques for Mobile Robot Trajectory Tracking

This paper presents a performance comparison of different estimation and prediction techniques applied to the problem of tracking multiple robots. The main performance criteria are the magnitude of the estimation or prediction error, the computational effort and the robustness of each method to non-Gaussian noise. Among the different techniques compared are the well known Kalman filters and their different variants (e.g. extended and unscented), and the more recent techniques relying on Sequential Monte Carlo Sampling methods, such as particle filters and Gaussian Mixture Sigma Point Particle Filter.

==> abbrev.tex <==
% Mathematical Reviews - AMS Abbreviations
% http://www.ams.org/msnhtml/serials.pdf
% http://www.ams.org/tools

% List of Serials
%
%Applied Mathematics and Optimization. An International Journal with Applications to Stochastics. Springer, New York. ISSN 0095-4616.
%
%Automatica. A Journal of IFAC, the International Federation of Automatic Control. Pergamon, Oxford. ISSN 0005-1098.
% * Communications on Pure and Applied Mathematics
%Computer Physics Communications. An International Journal and Program Library for Computational Physics and Physical Chemistry. North-Holland, Amsterdam. ISSN 0010-4655.
%
%European Journal of Control. Hermes Sci. Publ., Paris. ISSN 0947-3580.
%
%IEEE -- Institute of Electrical and Electronics Engineers -- 
%IEEE Transactions on Automatic Control. IEEE, Piscataway, NJ. ISSN 0018-9286.
%IEEE Transactions on Image Processing. IEEE, Piscataway, NJ. ISSN 1057-7149.
%IEEE Transactions on Information Theory. IEEE, Piscataway, NJ. ISSN 0018-9448.
%IEEE Transactions on Signal Processing. IEEE, Piscataway, NJ. ISSN 1053-587X.
%
%IMHOTEP. Journal Africain de M´athematiques Pures et Appliqu´ees. African Journal of Pure and Applied Mathematics. IMHOTEP Afr. J. Pure Appl. Math., Orl´eans.
%
%International Journal of Control. Taylor & Francis, London. ISSN 0020-7179.
%
%Journal of Differential Equations. Academic Press, Orlando, FL. ISSN 0022-0396.
%
%Journal of Functional Analysis. Academic Press, Orlando, FL. ISSN 0022-1236.
%
%Mathematics of Control, Signals, and Systems. Springer, Godalming. ISSN 0932-4194.
%
%Memoirs of the American Mathematical Society. Amer. Math. Soc., Providence, RI. ISSN 0065-9266.
%SIAM Journal on Control and Optimization. SIAM, Philadelphia, PA. ISSN 1095-7138.
%SIAM Review. SIAM, Philadelphia, PA. ISSN 1095-7200.
%
%Systems & Control Letters. North-Holland, Amsterdam. ISSN 0167-6911.
%
%* Zeitschrift f\"{u}r Wahrschichte Verw. Gebiete. 
%
%List of Proceedings
%IFAC Proc. Ser. IFAC Proceedings Series. IFAC, Laxenburg.
%Proceedings of the American Mathematical Society. Amer. Math. Soc., Providence, RI. ISSN 0002-9939.


% Abbreviations
% * Denotes not in Mathematical Reviews - AMS Abbreviations.
% Journals
\def\AMO{Appl. Math. Optim.}
\def\AUTOM{Automatica J. IFAC}

\def\COMMPAM{Commun. Pure Appl. Math.} %*
\def\COMPPHYS{Comput. Phys. Comm.}

\def\EJC{Eur. J. Control}

\def\IEEEAC{IEEE Trans. Automat. Control}
\def\IEEEIP{IEEE Trans. Image Process.}
\def\IEEEIT{IEEE Trans. Inform. Theory}
\def\IEEESP{IEEE Trans. Signal Process.}

\def\IMHOTEP{IMHOTEP J. Afr. Math. Pures Appl.}

\def\IJC{Internat. J. Control}

\def\JDE{J. Differential Equations}
\def\JFA{J. Funct. Anal.}
\def\MCSS{Math. Control Signals Systems}

\def\AMSM{Mem. Amer. Math. Soc.}

\def\SIAMCON{SIAM J. Control Optim.}
\def\SIAMREV{SIAM Rev.}
\def\SYSCON{Systems Control Lett.} 

\def\ZWV{Z. Wahrsch. Verw. Gebiete} %*

% Proceedings
\def\ACC{American Control Conf.}
\def\CDC{IEEE Conf. on Decision and Control}
\def\ICIP{IEEE Int. Conf. on Image Process.}
\def\IFAC{IFAC Proc. Ser.}
\def\AMSP{Proc. Amer. Math. Soc.}
\def\IEEEP{Proc. of the IEEE}
